BioSimulator.jl: Stochastic simulation in Julia

Biological systems with intertwined feedback loops pose a challenge to mathematical modeling efforts. Moreover, rare events, such as mutation and extinction, complicate system dynamics. Stochastic simulation algorithms are useful in generating time-evolution trajectories for these systems because they can adequately capture the influence of random fluctuations and quantify rare events. We present a simple and flexible package, BioSimulator.jl, for implementing the Gillespie algorithm, $\tau$-leaping, and related stochastic simulation algorithms. The objective of this work is to provide scientists across domains with fast, user-friendly simulation tools. We used the high-performance programming language Julia because of its emphasis on scientific computing. Our software package implements a suite of stochastic simulation algorithms based on Markov chain theory. We provide the ability to (a) diagram Petri Nets describing interactions, (b) plot average trajectories and attached standard deviations of each participating species over time, and (c) generate frequency distributions of each species at a specified time. BioSimulator.jl's interface allows users to build models programmatically within Julia. A model is then passed to the simulate routine to generate simulation data. The built-in tools allow one to visualize results and compute summary statistics. Our examples highlight the broad applicability of our software to systems of varying complexity from ecology, systems biology, chemistry, and genetics. The user-friendly nature of BioSimulator.jl encourages the use of stochastic simulation, minimizes tedious programming efforts, and reduces errors during model specification.

==> results.tex <==
\section{Results}

To illustrate the workflow of \pkg{BioSimulator.jl}, we provide three simple numerical examples using the SAL method unless otherwise specified.
In each case, we set $\epsilon = 0.03$, $\delta = 2$, and $\beta = 0.75$.

\input{example_kendall}
\input{example_mmek}
\input{example_autoreg}

\subsection{Algorithm comparison}

Here we compare the performance of \pkg{BioSimulator.jl}'s algorithms across the three examples from the previous sections.
Each model is simulated using the same model parameters outlined in the previous examples.
Each simulation task involves generating $100$ realizations.
In the case of fixed-interval output, $1000$ epochs are used.
The $\tau$-leaping algorithms use the default values $\epsilon = 0.03$, $\delta = 2$, and $\beta = 0.75$.

Table~\ref{tab:biosimulator-benchmarks} records the \textit{averaged} clock times reported by the \code{@benchmark} macro from \proglang{Julia}'s \pkg{BenchmarkTools.jl} package.
Each simulation task is allotted $2$ minutes to generate $100$ samples of the running time.
To be explicit, this means that the following command is executed \textit{at most} $100$ times:
\begin{minted}[fontsize=\scriptsize,samepage]{julia}
  simulate(model, algname, output_option, time = tfinal, epochs = 1000, trials = 100)
\end{minted}
Thus, these benchmarks reflect both the cost of generating a single realization, the efficiency of completing a typical simulation task, and the economy of choosing fixed-interval versus full simulation output.
Results are based on a MacBook Pro with 2 GHz Intel Core i7 (4 cores) and 16 GB of RAM running macOS High Sierra 10.13.3.
\begin{table}[!htbp]
  \centering
  \ra{1.3}
  \begin{tabular}{@{}cccc@{}}
    \toprule
    Algorithm & Kendall's process & Michaelis-Menten & Auto-regulation \\
    \midrule
    \multirow{2}{*}{SSA}
      & $1.04\ (1.03 - 1.05)$ & $0.783\ (0.788 - 0.808)$ & $426\  (424 - 432)$ \\
      & $1.38\ (1.37 - 1.40)$ & $0.918\ (0.909 - 0.936)$ & $1809\ (1734 - 1860)$ \\
    \midrule
    \multirow{2}{*}{FRM}
      & $1.04\ (1.03 - 1.05)$ & $0.863\ (0.853 - 0.874)$ & $464\  (462 - 468)$ \\
      & $1.35\ (1.33 - 1.37)$ & $0.983\ (0.973 - 1.000)$ & $1597\ (1408 - 1645)$ \\
    \midrule
    \multirow{2}{*}{NRM}
      & $2.72\ (2.71 - 2.75)$ & $3.11\ (3.08 - 3.15)$ & $1589\ (1581 - 1597)$   \\
      & $2.99\ (2.96 - 3.02)$ & $3.28\ (3.25 - 3.33)$ & $2724\ (2553 - 2775)$ \\
    \midrule
    \multirow{2}{*}{ODM}
      & $1.02\ (1.01 - 1.03)$ & $0.839\ (0.820 - 0.853)$ & $409\  (407 - 412)$ \\
      & $1.34\ (1.32 - 1.37)$ & $0.952\ (0.946 - 0.967)$ & $1648\ (1437 - 1721)$ \\
    \midrule
    \multirow{2}{*}{OTL}
      & $0.722\ (0.715 - 0.726)$ & $1.50\ (1.49 - 1.52)$ & $1867\ (1863 - 1877)$  \\
      & $0.754\ (0.751 - 0.760)$ & $1.64\ (1.63 - 1.67)$ & $3038\ (2845 - 3087)$ \\
    \midrule
    \multirow{2}{*}{SAL}
      & $0.596\ (0.588 - 0.599)$ & $0.989\ (0.985 - 0.996)$ & $1422\ (1415 - 1441)$  \\
      & $0.607\ (0.604 - 0.612)$ & $0.957\ (0.954 - 0.967)$ & $2578\ (2398 - 2631)$ \\
    \bottomrule
  \end{tabular}
  \caption{Median runtimes and interquantile ranges (in milliseconds) for Example 1, Example 2, and Example 3 based on $1000$ samples of the \code{simulate} command.
  Each simulation task generates $10$ realizations of the underlying stochastic model.
  For example, the median time to generate $10$ realizations of \textit{Kendall's process} using SSA is $1.04$ milliseconds.
  The first row in a cell is the benchmark result using the \code{Val(:fixed)} option for fixed-interval output.
  The second row indicates the timing result using the \code{Val(:full)} option for full simulation output.
  \label{tab:biosimulator-benchmarks}}
\end{table}

The NRM performs the worst across the selected model.
However, we note that \pkg{BioSimulator.jl} uses the a priority queue implementation from the \pkg{DataStructures.jl} package which may not be optimal for the method's specific demands.
Moreover, we take a na\"ive approach to building dependency graphs.
The overhead from \pkg{BioSimulator.jl}'s dependency graphs is sufficiently large that in some cases most of the simulation is spent on this step.
This warrants further review of our NRM implementation, although we expect an improved implementation to perform similarly to the FRM.
Only the auto-regulation model may show improved performance for the NRM over SSA because the reaction channels for that model are not tightly coupled.
Similarly, our ODM implementation may be inefficient based on its performance on the birth-death-immigration process.

Both $\tau$-leaping algorithms perform poorly on the auto-regulation model.
This is to be expected because neither OTL nor SAL handle separate time scales.
Figure~\ref{fig:autoreg}b shows that RNA transcription becomes a rare event as the protein dimer population grows.
Similarly, the free and blocked gene copies are always present in relatively small quantities compared to the protein and protein dimer populations.
Thus, protein dimerization and dissociation become the dominant reaction channels further along the time axis.
These two reactions drive the dynamics of the system and therefore heavily influence the $\tau$-leap selection procedure.
A natural consequence is that $\tau$-leaping methods have an increased likelihood of violating the leap condition in this regime and therefore bias the simulation toward infeasible states.
This assertion is easily verified using the \code{track_stats = true} option and checking the number of negative excursions reported by \pkg{BioSimulator.jl}.
In fact, the leap condition violations are egregious to the point that the recovery mechanism requires thinning the leap several times per negative excursion.
This suggests that reducing the leap size via the $\epsilon$ control parameter is likely to reduce the algorithm to SSA because leaps eventually become smaller than the expected Gillespie updates.

\subsection{Software comparison}

We compare \pkg{BioSimulator.jl}'s features and performance against three software packages: \pkg{StochPy}, \pkg{StochKit2}, and \pkg{Gillespie.jl}.
The tools in the space of stochastic simulation are manifold and vary in their features and applications.
Naturally, there are many omissions.
Each software package is selected for its similarity to \pkg{BioSimulator.jl}.
Specifically, these tools are domain-independent, general purpose Gillespie-like simulators.
Table~\ref{table:soft-compare} summarizes the differences and similarities between these software tools.
\begin{table}
  \centering
  \ra{1.3}
  \begin{tabular}{@{}rccccccc@{}}
    \toprule
    & \pkg{StochPy} & \pkg{StochKit2} & \pkg{Gillespie.jl}     & \pkg{BioSimulator.jl} \\
    \midrule
    \textbf{Software characteristics}: & & & & \\
    Language & Python  & C++       & Julia            & Julia \\
    Open-source & Yes & Yes & Yes & Yes \\
    GUI & No & via StochSS & No & No \\
    Jupyter integration & Yes & No & Yes & Yes \\
    Performance & Fast & Faster & Faster & Fastest \\
    \textbf{Interactivity}: &     &             &     & \\
    Model editor            & No  & via StochSS & No  & Yes \\
    Simulation interface    & Yes & via StochSS & Yes & Yes \\
    Plotting         & Yes & Limited & No & Yes \\
    \textbf{Simulation features}: & & & & \\
    Fixed-interval output & via StochKit2 & Yes & No & Yes \\
    Full output & Yes & Yes & Yes & Yes \\
    SBML support & Yes & Yes & No & No \\
    Readable input & Yes & No & No & Yes \\
    Parallelism & No & Yes & No & Yes \\
    \bottomrule
  \end{tabular}
  \caption{A summary of features across \pkg{StochPy}, \pkg{StochKit2}, \pkg{Gillespie.jl}, and \pkg{BioSimulator.jl}. Jupyter notebooks are human-readable documents that combine code, text, and figures into a single interactive report.}
  \label{table:soft-compare}
\end{table}

In addition, we compare each software package on simulation speed across five different models:
\begin{enumerate}[label=(\alph*)]
  \item \textit{Kendall's process} permits an analytic mean trajectory.
  This model serves as an easy speed test and a correctness check.

  \item The \textit{Michaelis-Menten enzyme kinetics} model provides a second simple speed test with multiple species.

  \item The \textit{auto-regulation} model serves a benchmark against an interesting biological application of stochastic simulation.

  %%%% cite a paper for the model %%%%
  \item The \textit{dimer-decay} model is an example of a small stiff system.
  It is featured in the literature as a $\tau$-leaping benchmark \citep{efficient,slow-scale-tau}.

  %%%% cite a paper for the model %%%%
  \item A \textit{yeast} model from biology is another interesting stiff system used here as a benchmark. \citep{chou2008,drawert2010,yeast-biology}.
\end{enumerate}
Initial conditions and other model parameters are deferred to supplementary information (Section A.1, Tables S1 - S5).
Table~\ref{tab:benchmarks} reports the benchmark results and includes the \textit{simulation} parameters.

\begin{landscape}
\begin{table}[!htbp]
\centering
\centering
\ra{1.3}
\begin{tabular}{@{}crrrrr@{}}
    \toprule
    Software & \multicolumn{1}{c}{\pkg{StochPy}} & \multicolumn{1}{c}{\pkg{StochKit2}} & \multicolumn{1}{c}{\pkg{Gillespie.jl}} & \multicolumn{2}{c}{\pkg{BioSimulator.jl}} \\
    Method   & \multicolumn{1}{c}{SSA}           & \multicolumn{1}{c}{SSA (dep. graph)}             & \multicolumn{1}{c}{SSA}                & \multicolumn{2}{c}{SSA} \\
    Mode     & \multicolumn{1}{c}{Serial}        & \multicolumn{1}{c}{Parallel}        & \multicolumn{1}{c}{Serial}             & \multicolumn{1}{c}{Serial} & \multicolumn{1}{c}{Parallel} \\
    \midrule % biosimulator is currently in ms
    \multirow{2}{*}{Kendall's process}
      &                    & $174.31\ (173.81 - 174.95)$ &                       & $1.04\ (1.03 - 1.05)$ & $0.56\ (0.48 - 0.66)$ \\
      & $257\ (223 - 296)$ &                             & $1285\ (1280 - 1293)$ & $1.38\ (1.37 - 1.40)$ & $0.79\ (0.68 - 0.93)$ \\
    \multirow{2}{*}{Michaelis-Menten}
      &                    & $210.42\ (209.89 - 211.14)$ &                       & $0.783\ (0.788 - 0.808)$ & $0.45\ (0.44 - 0.46)$ \\
      & $214\ (213 - 216)$ &                             & $1.15\ (1.12 - 1.21)$ & $0.918\ (0.909 - 0.936)$ & $0.47\ (0.46 - 0.48)$ \\
    \multirow{2}{*}{Auto-regulation}
      &                                      & $432\ (425 - 445)$ &                    & $426\  (424 - 432)$ & $135\ (124 - 149)$ \\
      & $8.23\ (7.87 - 8.75); \times 10^{4}$ &                    & $824\ (762 - 834)$ & $1809\ (1734 - 1860)$ & $211\ (193 - 240)$ \\
    \multirow{2}{*}{Dimer-decay}
      &                    & $216.98\ (216.52 - 217.68)$ &                       & $1.76\ (1.75 - 1.79)$ & $0.81\ (0.80 - 0.82)$ \\
      & $483\ (480 - 488)$ &                             & $2.68\ (2.66 - 2.84)$ & $2.39\ (2.37 - 2.42)$ & $1.03\ (1.02 - 1.05)$ \\
    \multirow{2}{*}{Yeast}
      &                    & $260\ (254 - 267)$ &                       & $2.56\ (2.53 - 2.63)$ & $1.38\ (1.10 - 1.42)$ \\
      & $469\ (465 - 474)$ &                    & $2.25\ (2.21 - 2.63)$ & $2.92\ (2.89 - 2.99)$ & $1.24\ (1.20 - 1.27)$ \\
    \bottomrule
\end{tabular}
\caption{Median runtimes and interquantile ranges for \pkg{StochPy}, \pkg{StochKit2}, \pkg{Gillespie.jl}, and \pkg{BioSimulator} across selected models based on $1000$ samples, reported in milliseconds (ms).
Each sample measured the time to generate $10$ realizations of a given stochastic process.
Results using fixed-interval and fixed output options are recorded in the first and second rows of each cell, respectively.
Each simulation tool is used with its default settings.
For example, \pkg{StochKit2} automatically parallelizes simulation tasks involving multiple realizations and uses a dependency graph by default.
We note that both \pkg{StochKit2} and \pkg{BioSimulator.jl} used $8$ threads for the parallel simulation benchmarks.
Direct comparisons based on these results are not possible, in the sense that slower performance does not necessarily indicate a particular tool is poorly implemented.
Rather, our results reflect natural trade-offs in optimizing software for particular goals.
\textbf{Note}: The \pkg{StochPy} benchmark on the \textit{auto-regulation} model is based on only $100$ samples.
\label{tab:benchmarks}}
\end{table}
\end{landscape}

\subsection{Package availability}

\pkg{BioSimulator.jl} is available on GitHub (\url{https://github.com/alanderos91/BioSimulator.jl}).
All source code is readily available to view, download, and distribute under the MIT license.
We also maintain a documentation manual via GitHub Pages (\url{https://alanderos91.github.io/BioSimulator.jl/stable/}).

